A Hierarchical N-Gram Framework for Zero-Shot Link Prediction

Due to the incompleteness of knowledge graphs (KGs), zero-shot link prediction (ZSLP) which aims to predict unobserved relations in KGs has attracted recent interest from researchers. A common solution is to use textual features of relations (e.g., surface name or textual descriptions) as auxiliary information to bridge the gap between seen and unseen relations. Current approaches learn an embedding for each word token in the text. These methods lack robustness as they suffer from the out-of-vocabulary (OOV) problem. Meanwhile, models built on character n-grams have the capability of generating expressive representations for OOV words. Thus, in this paper, we propose a Hierarchical N-Gram framework for Zero-Shot Link Prediction (HNZSLP), which considers the dependencies among character n-grams of the relation surface name for ZSLP. Our approach works by first constructing a hierarchical n-gram graph on the surface name to model the organizational structure of n-grams that leads to the surface name. A GramTransformer, based on the Transformer is then presented to model the hierarchical n-gram graph to construct the relation embedding for ZSLP. Experimental results show the proposed HNZSLP achieved state-of-the-art performance on two ZSLP datasets.

==> introduction_back.tex <==


\section{Introduction}
%Typically, these models aim to predict a tail entity given a head entity and a query relation.
Link prediction models aim to predict relations between entities in knowledge graphs.  The success of these models however depend on their ability to learn expressive representations for entities and relations that preserve the structure of the knowledge graph~\cite{sun2019rotate,chen2020hitter}. Traditional approaches~ \cite{bordes2013translating} assume that all relation types are known in the KG. This assumption is however unrealistic since KGs are inherently incomplete. Learning link prediction models that can deal with unseen relations has thus become of great importance in KG research communities. To facilitate research, the zero-shot link prediction task has been introduced to predict unseen relations by leveraging auxiliary information that bridges the gap between seen and unseen relations~\cite{qin2020generative}.  %~\cite{xian2018zero,romera2015embarrassingly,xian2017zero}.  %Thus, which ultimately helps solve the task of zero-shot link prediction, where the goal is to predict relations between entities that are unobserved during training.

\begin{table}[ht!]
    \centering
    \small
    \begin{tabular}{l|l}
    & {\bf Relation:} ``{\tt teammate}'' \\ \hline
      \bf Wikidata  &  A person in one's team\\
      \bf NELL  & Two athletes are teammates if they play on \\
      & the same team
    \end{tabular}
    \caption{Two sources with different nuances in the definition (or textual description) for the relation {\tt teammate}}.
    \label{tab:teammate}
\end{table}

%As like \cite{qin2020generative},  \citet{geng2021ontozsl} considers the textual descriptions of relations and additionally learns the ontology for relations.

Little research has been performed on zero-shot link prediction as the task is relatively new~\cite{qin2020generative,geng2021ontozsl,wang2021structure}. Recent efforts have been devoted to utilizing textual features~\cite{qin2020generative,wang2021structure} or ontology~\cite{geng2021ontozsl} as auxiliary information for the task. Particularly, while \citet{wang2021structure} use surface names of entities and relations, \citet{qin2020generative} use the textual descriptions of relations.  Though driven by a common motivation, that is, seen and unseen relations may share word or character information for zero-shot learning, using textual descriptions at present may give rise to key issues as we will see shortly.

% To better utilize knowledge graphs in downstream applications,  knowledge graph embedding (KGE) has been introduced to represent entities and relations in KGs~\cite{sun2019rotate,chen2020hitter}. The traditional KGE task assumes that all relation types are known in the KG. This assumption is however unrealistic since KGs are inherently incomplete. Learning KGE models that can deal with unseen relations has thus become of great importance in KG research communities. To facilitate research, zero-shot learning (ZSL) \cite{xian2018zero,romera2015embarrassingly,xian2017zero} has been introduced in KGE to bridge the gap between seen and unseen relations through some form of auxiliary information such as the textual descriptions of relations~\cite{qin2020generative}.

%Zero-shot learning (ZSL) \cite{xian2018zero,romera2015embarrassingly,xian2017zero} is such an approach that can be introduced in KGE to tackle the unseen-relation problem.



% A recent task that utilizes zero-shot learning into KGE is zero-shot link prediction. Several models for this task have been proposed in research community, such as ZSGAN \cite{qin2020generative} and OntoZSL~\cite{geng2021ontozsl}.

% A recent task that has benefited from zero-shot KGE is zero-shot link prediction. Briefly, zero-shot link prediction aims to predict relations between entities that are unobserved during training. The typical approach is to predict a tail entity given a head entity and a query relation. As this task is relatively new, only few works have been proposed so far~\cite{qin2020generative,geng2021ontozsl,wang2021structure}. Notably, these methods learn the word token information from the external textual descriptions of relations~\cite{qin2020generative,wang2021structure} or ontology~\cite{geng2021ontozsl} to bridge the gap between seen or unseen relations for the task.

% Among them, ZSGAN~\cite{qin2020generative}  proposes to generate the unseen relation representations from textual descriptions of relations by utilizing generative adversarial networks (GAN)~\cite{goodfellow2014generative}. OntoZSL introduces an ontological schema~\cite{guarino1995formal} to pre-train on an external ontology to obtain the structural information of unseen relations. Otherwise, STAR~\cite{wang2021structure} utilizes the language model to infer the tail entity by utilizing textual information from entities and relations. 



First, textual descriptions of relations are often unaccompanied with prevailing knowledge graphs (e.g., WordNet~\cite{miller1995wordnet}, FreeBase~\cite{bollacker2008freebase}). As such, current methods that utilize textual descriptions obtain them from external sources. But these external sources may have different nuances in their word definitions for certain relations which may lead to unreliable results. For example, consider the relation ``{\tt teammate}'' and its definition provided by different knowledge bases as shown in Table~\ref{tab:teammate}. The NELL definition may require that the entities in a ``{\tt teammate}'' relationship are athletes if we are to learn a semantic representation on its textual description. On the other hand, Wikidata's definition is more general and covers the definition of ``{\tt teammate}'' more appropriately. Unfortunately, there are no automatic means to collect the best suited textual descriptions of relations for the task, which makes the process labor-intensive and time-consuming. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth]{figure1.pdf}
	\caption{Overview of our proposed approach. Through building the lattice graph for the surface name of relation, and calculating the lattice graph information by Graph encoder module, we can get the semantic representation for the relation. In the testing progress, the trained KGE model and Graph encoder model can be used to 
	to generate reasonable embeddings for unseen relations and predict the new tail entity. $H_t$ refers the embedding of head entity in the training progress.\ref{con:overview of our method}.
	}
	\label{Figure 1}
	\label{con:overview of our method}
\end{figure}

Alternatively, \citet{wang2021structure} introduced a language model~\cite{liu2019roberta} to learn a word representations on the surface name of relations. As surface names are readily available in the KG, this approach is more robust. However, the approach proposed in this work faces two fundamental weakness. Firstly, context is an essential requirement for any text representation method or zero-shot learning. Surface names on the other hand are represented by short texts, e.g., the relation ``{\tt teammate}'' will have a single word representation observed in training and will therefore have little to no association with an unobserved relation for zero-shot. Secondly, the language model lack the ability to capture representations for out-of-vocabulary words. This same problem also applies to models that aim to learn from textual descriptions of relations. In such cases,
the relation representation ability of current methods may be limited significantly, which inadvertently hurts the zero-shot link prediction performance. 

% Despite their success, some models heavily rely on external auxiliary information, including textual descriptions of relations~\cite{qin2020generative} or ontology~\cite{geng2021ontozsl} which are often unaccompanied with prevailing knowledge graphs (e.g., WordNet~\cite{miller1995wordnet}, FreeBase~\cite{bollacker2008freebase}). 

% One obvious drawback is that, entities and relations may have heterogeneous textual descriptions from different external sources which may lead to unreliable link prediction results. Besides, there are no automatic means to collect the best suited descriptions of entities/relations for the task, which makes the process labor-intensive and time-consuming.
%%%%%%%%%
% To solve this problem, some works such as ~\cite{wang2021structure} that use language model to learn the surface name information of relation, this surface name information is easy to obtain. However, Either some works use textual description information or surface name information of relations to learn the relation representation,
% % Then again, existing works such as \cite{geng2021ontozsl,wang2021structure} that 
% they all use word embeddings to represent these textual information may suffer from out-of-vocabulary problem, where some unknown words appear in the descriptions or surface name. The above mentioned problems may limit the performance of existing zero-shot link prediction models. 

% these models rely on  hardly collected external resources, such as textual descriptions of relations or ontology, which are usually not provided. For example, Commonly used knowledge graphs, such as WordNet~\cite{miller1995wordnet}, FreeBase~\cite{bollacker2008freebase}, do not includes the textual description of relations and ontology. Furthermore, existing works utilizing the word embedding to represent text descriptions may suffer from out-of-vocabulary problem when some undefined words appear in the descriptions. The above mentioned problems may limit the performance of existing zero-shot link prediction models.

% More importantly, the prior works haven't explored the lattice information of surface name, which may further boost the zero-shot learning performance.

Without adopting external textual descriptions or simply learning word representations from surface name relations, we show it is possible to learn expressive relation representations on surface names for the problem at hand. The core premise of our approach is that while the formation of words are to some extent sequence-like, thus, the sequential combination of characters or n-grams, it can be visualized as a hierarchical structure from the sequential combination of single characters or going down to different levels of sequential combination of n-grams. We refer to this combinational n-gram/character structure as a lattice graph. In this case, a relational lattice graph given that we intend to construct a lattice from the surface name of the relation. 

Figure~\ref{Figure 1} illustrates the lattice graph for the seen relation ``{\tt has}'' and unseen relation ``{\tt as}'' in the overview of our approach.

% A straightforward strategy is to learn and aggregate the word embeddings of relation surface names to construct the relation representation. However, surface names lack contextual information of the target relation, which makes it difficult to obtain a semantic-rich relation representation. 

%Instead of incorporating expensive external resources, in this work, we attempt to represent the relations with easily accessed surface names. As surface names lack of contexts about the target relations, it is difficult to obtain semantic-rich relation representations using the word embedding of surface names. 
To effectively utilize surface names in relation representation and avoid out-of-vocabulary problem, we propose to use hybrid N-Gram to divided the sentence, this way can
make sure almost all testing n-gram blocks will be in the training n-gram blocks, so the zero-shot learning problem can be change into a surprised learning, and the out-of-vocabulary problem will be solved, at the same time, the hybrid n-gram information also can provide rich contextual information for each gram.


For the ordinary way to capture the context information of each gram is to build the fully connected graph, by this way the gram can choose the most important grams to help calculate its information.
% the n-gram information is to regard  the grams as a list, and then capture the gram information based on its context. For example, in relation \textit{"has"}, the n-grams are 
% \textit{"h,a,s,ha,as,has"}. 
% %%%%%%%%%
% By researching, we found it is difficult to set the context window to learn the gram context information, if we set the window size is 2, the context of "as" is "s" and "ha", but gram "a" has the connection with "as", because they all have "a". 
% The best way to solve this issue is to build the fully connected graph, by this way the gram can learn the relationships for other grams. 
However this method cannot learn the specific information for two grams, for example, in relation \textit{"has"}, the n-grams are \textit{"h,a,s,ha,as,has"},  the weight value between "a" and "as" should bigger than the weight value between "h" ans "as", even "a" and "h" all connect to "as", because "as" and "a" all have "a". The machine will make a mistake to  assign the weight value, because the machine  does know the connection for  "as" and "a".

So, in our work, we propose to use lattice graph \footnote{In our work, the lattice refers to n-gram block, for the detail, please check Section \ref{con:detail of lattice graph}}, to help model learn the right context and relationship information, which has shown its power in semantic representation by encoding the character-structure of words~\cite{tay2021charformer}.
% but we found when we learn this information, the current work \cite{tay2021charformer} encoder all relation in the graph in the same semantic space, while as suggest in~\cite{cai2020graph,fu2020magnn}, it is not ideal as different types information are typically same elements. 
%%%%%%%%%%%%%%%%
% \textcolor{red}{
When we calculate the lattice graph information,
We found the node in the lattice graph information is from different direction (one lattice connects two different type relation information), such as in Figure~\ref{con:overview of our method}, the information of lattice node $a$ is from its neighbor node $h$ (internal nodes) and its composition node $ha$ (external nodes). 
% So, in our work, we build the lattice graph for each relation surface name to help encoder  above information, the lattice graph for relation "has" is shown in Figure.\ref{con:overview of our method}, for the detail about lattice graph, please refer section \ref{con:detail of lattice graph}.

% \textcolor{red}{However, existing lattice encoding methods suffer two challenges which limits its application to zero-shot link prediction. To achieve this goal, prior works~\cite{tay2021charformer, xue2021byt5} regard the characters \footnote{The characters of word $at$ are $a$ and $t$.} as the lattices, and use the attention-based methods to learn the semantic representation of characters . However, this method cannot be used to calculate the information of lattice which has more than one character, for example, learning the information about $t$ and $a$ cannot represent the semantic information about $at$ and $ta$ even with the positional encoding since they have different contexts. To solve this problem, we utilize the n-gram method to decompose surface name, and regard the gram as the lattice, by this way, the model can learn the information about lattice correctly which includes more than one character. }
%%%%%%%%%%




\textcolor{red}{So the main challenge is how to build a lattice encoder model which is capable of calculating richer node information  and transferring correlation among the seen relations to the unseen relations for zero-shot link prediction.}

\textcolor{red}{In this paper, we propose a novel ZSL method called LZSL, a \textbf{L}attice framework for \textbf{Z}ero \textbf{S}hot \textbf{L}ink prediction, since the "Lattice" in our method refers to the lattice information. The whole progress is shown in Figure~\ref{con:overview of our method}.
In the first step of our work, we build a lattice graph for each relation base on its surface name, 
% Unlike current work~\cite{zhang2020relational} that use GCNs to model the graph information, 
and explore the attention mechanism in Transformer~\cite{vaswani2017attention} to model the graph information. 
% since each node has positional information and we need to build the node information based on different relation information.
Transformer is responsible for learning the correlations between each node using self-attention mechanisms. We however improve the attention mechanism by including internal node information, external node information and two different type relation information to encourage the Transformer to attend to all the important nodes from different vector space based on the relation information when constructing an embedding for the unseen relations.}

\textcolor{red}{Our  treatment of node encoding and relation encoding bring advantages compared to the methods which use Graph Convolutional Network (GCN) to model the graph information. Previous, the state-of-the-art GCN graph modeling method ~\cite{zhang2020relational} regard the relations also as the nodes, for example, for two node ( h and a) in our lattice graph, the relation for these two nodes is "neighbor", so the triple is (h, neighbor, a), this labeled edge turns to be two unlabeled edges (h, neighbor) and  (neighbor,a). The relation and entity node will share the same semantic space. This way is not ideal as relation and entity are typically different elements. In addition, in the lattice graph different relations are also different elements, they can not be encoded in the same semantic space. Through internal node encoder, external node encoder and their relevant relation encoder, our LatticeTransformer can avoid these problems.}
% We refer to this  architecture as LatticeTransformer.
%We then propose a structure-aware embedding module  that learns a transferable score function for the unseen relations.

% To demonstrate the effectiveness of our approach, we evaluate our approach on the zero-shot link predictions. 
% Moreover, we design a simple approach to integrate LatticeTransformer into the pre-trained model BERT and show its effectiveness on zero shot triple classification. To the best of our knowledge, our work is the first to utilize the lattice graph information for the ZSL triple classification task. 
% It uses a Lattice Transformer model to learn the representation of each node in lattice graph we build, by aggregating information from different graph neighbors. Although prior work show that Transformers can learn the graph information from the textual data \cite{cai2020graph,ahmad2021gate}, it is not ideal as different types relation are mapped in a same vector space. Lattice Transformer explicitly operates the nodes over structure input using different relation information.
The main contributions of this paper are summarized as follows:
\begin{itemize}
	\item We propose a novel framework LZSL which using the lattice information from relation surface name to solve the zero shot link prediction task. No additional resources required.
	
	\item We propose a novel LatticeTransformer to encoder the different types node and relation information in the lattice graph.
	
	\item Extensive experiments on two zero-shot datasets of link prediction  show that our method significantly outperforms prior state-of-the-art methods.
\end{itemize}
